Conditional Contrastive Learning with Kernel

Conditional contrastive learning frameworks consider the conditional sampling procedure that constructs positive or negative data pairs conditioned on specific variables. Fair contrastive learning constructs negative pairs, for example, from the same gender (conditioning on sensitive information), which in turn reduces undesirable information from the learned representations; weakly supervised contrastive learning constructs positive pairs with similar annotative attributes (conditioning on auxiliary information), which in turn are incorporated into the representations. Although conditional contrastive learning enables many applications, the conditional sampling procedure can be challenging if we cannot obtain sufficient data pairs for some values of the conditioning variable. This paper presents Conditional Contrastive Learning with Kernel (CCL-K) that converts existing conditional contrastive objectives into alternative forms that mitigate the insufficient data problem. Instead of sampling data according to the value of the conditioning variable, CCL-K uses the Kernel Conditional Embedding Operator that samples data from all available data and assigns weights to each sampled data given the kernel similarity between the values of the conditioning variable. We conduct experiments using weakly supervised, fair, and hard negatives contrastive learning, showing CCL-K outperforms state-of-the-art baselines.

==> sec/archive/cond_sample_old.tex <==
\section{Conditional Sampling in Contrastive Learning}
\label{sec:cond_sample}
This section focuses on discussing the {\em conditional sampling procedure} in contrastive learning literature. In particular, we shall present the mathematical form of the conditional sampling, showing that it plays an important role in several contrastive approaches. For notations, we use uppercase letters (e.g., $X$) to denote random variables, $P_\cdot{\cdot}$ to denote the distribution (e.g., $P_X$ denotes the distribution of $X$), lowercase letters (e.g., $x$) to denote the outcome from a variable, and the calligraphy letter (e.g., $\mathcal{X}$) to denote the sample space of a variable.  
 
\subsection{Technical Preliminaries} 
The general idea behind contrastive learning is to learn similar representations for {\em positively-paired} data and dissimilar representations for {\em negatively-paired} data~\citep{tsai2021conditional,tsai2021integrating,chen2020simple,he2020momentum,hjelm2018learning}. Literature~\citep{oord2018representation,tsai2021self,bachman2019learning,hjelm2018learning} suggests that the construction of the positive and negative data pairs can be understood as the sampling procedure from data distributions. To see this, we begin by reviewing the most dominant contrastive approach - the InfoNCE objective~\citep{oord2018representation}:
\begin{equation}
\small{
{\rm InfoNCE}:=\underset{f}{\rm sup}\,\,\mathbb{E}_{(x,y_{\rm pos})\sim P_{XY}\,,\, \{y_{\rm neg,i}\}_{i=1}^n\sim {P_{Y}}^{\otimes n}} \Big[\,{\rm log}\,\frac{e^{f(x, y_{\rm pos})}}{e^{f(x, y_{\rm pos})} + \sum_{i=1}^n e^{f(x, y_{\rm neg,i})}}\Big],
}
\label{eq:infonce}
\end{equation}
where $X$ and $Y$ represent the data  {\color{olive} Martin: X and Y may not be data, but representations instead?} {\color{red} I'm intentionally making $X$ and $Y$ to be data but not representations.}, $x$ is the anchor data, $(x, y_{\rm pos})$ are positively-paired and are sampled from $P_{XY}$, $\{(x, y_{\rm neg, i})\}_{i=1}^n$ are negatively-paired and are sampled from $P_XP_Y$, and $f(\cdot, \cdot)$ defines a mapping $\mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}$. Same as most of the prior work~\citep{chen2020simple,he2020momentum}, we parametrize $f$ via neural networks with the following design:
\begin{equation}
    f(x,y) := {\rm cosine\,\,similarity} \Big(g_{\theta_X}(x), g_{\theta_Y}(y)\Big) / \tau,
\label{eq:f}
\end{equation}
where $g_{\theta_X}$ and $g_{\theta_Y}$ are neural networks ($g_{\theta_X}$ can be the same as $g_{\theta_Y}$) parameterized by parameters $\theta_X$ and $\theta_Y$, and $\tau$ is a hyper-parameter that rescales the score from the cosine similarity. With this design, taking supreme over $f$ in~\eqref{eq:infonce} can be regarded as performing gradient ascent over $\theta_X$ and $\theta_Y$. Then, the InfoNCE objective suggests to maximize the similarity score between a data pair sampled from the joint distribution  (i.e., $(x,y_{\rm pos})\sim P_{XY}$) and minimize the similarity score between a data pair sampled from the product of marginal distribution  (i.e., $(x,y_{\rm neg})\sim P_{X}P_{Y}$). 

We next look at an example that uses the InfoNCE objective - the SimCLR method~\citep{chen2020simple}. SimCLR considers augmented variants (by applying image augmentations) of the same image as positively-paired and different images as negatively-paired. For positively-paired images  $x$ and $y$, since they are augmented variants of the same image, they can be seen as different views to each other, as if they are sampling from the joint distribution of the data: $(x,y) \sim P_{XY}$. On the contrary, for negatively-paired images $x$ and $y$, since they are different images, they can be seen as sampling from the product of marginal distributions: $(x,y) \sim P_XP_Y$.




There are recent methods~\citep{robinson2020contrastive,wu2020conditional,tsai2021integrating,tsai2021conditional} that modify the InfoNCE objective, by sampling under certain conditions, to construct more suitable positive or negative pairs depending on their goals. We bring them under an umbrella called the {\em conditional sampling procedure}. In particular, defining $Z$ as the conditioned variable and $z$ as its outcome, the conditional sampling procedure samples the positive or negative data pairs from the product of conditional distribution: $(x,y)\sim P_{X|Z=z}P_{Y|Z=z}$, where $x$ and $y$ are sampled given the same value of the conditioned variable. Below, we discuss these methods, where they consider different conditioned variable types, such as distance to data~\citep{robinson2020contrastive,wu2020conditional}, auxiliary information~\citep{tsai2021integrating}, and sensitive information~\citep{tsai2021conditional}. To ease the presentation, we present their objectives in our own words but not strictly follow the original ones. 



%\cite{robinson2020contrastive,wu2020conditional} samples negatives that are harder  for $f$ to learn by conditioning on the current positive samples, to achieve better downstream performances.  \citet{tsai2021integrating} samples positive pairs conditioning on the same cluster (formed by auxiliary attribute) to integrate auxiliary information. And \citet{tsai2021conditional} samples negative pairs conditioning on the same sensitive attribute to remove undesirable sensitive information. 



\subsection{Hard-negative Contrastive Learning: Conditioning on Distance to Data}\label{method:hardnegatives}

\citet{robinson2020contrastive} and \citet{kalantidis2020hard} argue that learning contrastive representations benefits from hard negative samples (i.e., samples that are difficult to distinguish from an anchor sample). To this end, rather than considering arbitrary two random data as negatively-paired, these work considers to construct a negative data pair from two random data that are not too far from each other\footnote{\citet{wu2020conditional} argues a better construction of negative data pairs is selecting two random data that are neither too far nor too close to each other.}. To embrace this idea, the original InfoNCE objective in~\eqref{eq:infonce} is modified into the hard-negative InfoNCE (abbreviated as HardNeg-InfoNCE) objective:
\begin{equation}
\small{
\begin{split}
&{\rm HardNeg-InfoNCE}\\
&:=\underset{f}{\rm sup}\,\,\mathbb{E}_{(x,y_{\rm pos})\sim P_{XY}\,,\, z \sim P_{Z|X=x,Y=y_{\rm pos}} \,,\, \{y_{\rm neg,i}\}_{i=1}^n \sim P_{Y|Z=z}^{\otimes n}}\Big[\,{\rm log}\,\frac{e^{f(x, y_{\rm pos})}}{e^{f(x, y_{\rm pos})} + \sum_{i=1}^n e^{f(x, y_{\rm neg,i})}}\Big].
\end{split}
}
\label{eq:hard_infoNCE}
\end{equation}
$Z$ is the conditioned variable representing whether the distance is close to data $X$, so that $z$ represents an indicator of the closeness to the anchor data $x$. $(x, y_{\rm pos})$ are positively-paired that are sampled from $P_{XY}$. Note that we also assume $y_{\rm pos}$ is close to $x$, and hence $x$ and $y_{\rm pos}$ are associated with the same $z$. $\{(x, y_{\rm neg, i})\}_{i=1}^n$ are negatively-paired, where $\{y_{\rm neg, i}\}_{i=1}^n$ are sampled from the conditional distribution $P_{Y|Z=z}$. To be more specific, since we represent $z$ as the distance to data $x$, we refer the sampling $y \sim P_{Y|Z=z}$ as if selecting $y$ that are close to $x$. 

We also provide an alternative way to think of the hard negative sampling process. We can regard the conditioned variable $Z$ as a data point and re-express the negative-pair sampling procedure as $\{(x, y_{\rm neg, i})\}_{i=1}^n$ from $P_{X|Z=z}P_{Y|Z=z}$. Then, sampling from $P_{X|Z=z}P_{Y|Z=z}$ can be understand as sampling $x$ and $y$ that are close to the center $z$, resulting in the closeness between $x$ and $y$.
 

\subsection{Weakly-supervised Contrastive Learning: Conditioning on Auxiliary Information}

\citet{tsai2021integrating} presents a weakly-supervised representation learning method, which considers the auxiliary information from data (e.g., annotation attributes of images) as a supervision signal when learning representations. This work is motivated by the argument that the auxiliary information implies semantic similarities. With this motivation, the paper introduces a weakly-supervised contrastive learning framework that learns similar representations for data with the same auxiliary information and dissimilar representations for data with different auxiliary information. Embracing this idea, the original InfoNCE objective in~\eqref{eq:infonce} can be modified into the weakly-supervised InfoNCE (abbreviated as WeaklySup-InfoNCE) objective:
\begin{equation}
\small{
\begin{split}
&{\rm WeaklySup-InfoNCE}\\
&:=\underset{f}{\rm sup}\,\,\mathbb{E}_{z\sim P_Z\,,\, (x,y_{\rm pos})\sim P_{X|Z=z} P_{Y|Z=z} \,,\,\{y_{\rm neg,i}\}_{i=1}^n \sim P_{Y}^{\otimes n}} \Big[\,{\rm log}\,\frac{e^{f(x, y_{\rm pos})}}{e^{f(x, y_{\rm pos})} + \sum_{i=1}^n e^{f(x, y_{\rm neg,i})}}\Big].
\end{split}
}
\label{eq:weaksup_infoNCE}
\end{equation}
$Z$ is the conditioned variable representing the auxiliary information from data, and $z$ is the value of auxiliary information that we sample from $P_Z$. $(x, y_{\rm pos})$ are positively-paired that are sampled from $P_{X|Z=z}P_{Y|Z=z}$. By this design, the positively-paired samples are always having the same value of the conditioned variable. $\{(x, y_{\rm neg, i})\}_{i=1}^n$ are negatively-paired that are sampled from $P_XP_Y$.


\subsection{Fair Contrastive Learning: Conditioning on Sensitive Information}

Another recent work \citep{tsai2021conditional} presents to remove the sensitive information when learning contrastive representations, such as learning fair representations that can ignore the effect from gender or race. To reach this goal, the paper argues that in the contrastive learning framework, we should fix the value of the sensitive variable. {\color{olive} Martin: We may re-consider the following sentence as this is not very intuitive} {\color{red} Please fix it.} Since the value of the sensitive variable is fixed, we are ignoring the variations of the sensitive variable, and hence the effect from it would be removed. Embracing this idea, the original InfoNCE objective in~\eqref{eq:infonce} can be modified into the Fair-InfoNCE objective:
\begin{equation}
\small{
\begin{split}
&{\rm Fair-InfoNCE}\\
&:=\underset{f}{\rm sup}\,\,\mathbb{E}_{(x,y_{\rm pos})\sim P_{XY}\,,\, z\sim P_{Z|X=x, Y=y_{\rm pos}}\,,\,\{y_{\rm neg,i}\}_{i=1}^n \sim P_{Y|Z=z}^{\otimes n}}\Big[\,{\rm log}\,\frac{e^{f(x, y_{\rm pos})}}{e^{f(x, y_{\rm pos})} + \sum_{i=1}^n e^{f(x, y_{\rm neg,i})}}\Big].
\end{split}
}
\label{eq:fair_infoNCE}
\end{equation}
$Z$ is the conditioned variable representing the sensitive information (e.g., race), $z$ is the value of the sensitive information (e.g., Asian), and the anchor data $x$ that is associated with $z$ (e.g., a data point that falls in the Asian category). $(x, y_{\rm pos})$ are positively-paired that are sampled from $P_{XY}$. Note that, by construction, we assume $x$ and $y_{\rm pos}$ are associated with the same $z$. $\{(x, y_{\rm neg, i})\}_{i=1}^n$ are negatively-paired that are sampled from $P_{X|Z=z}P_{Y|Z=z}$. By this design, the positively-paired samples and the negatively-paired samples are always having the same value of the conditioned variable. %Note that we fix $Z=z$ for iteration but vary $z$ for different iterations.

\subsection{Comparisons between Different Sampling Procedures}

For the HardNeg-InfoNCE (\eqref{eq:hard_infoNCE}) and Fair-InfoNCE (\eqref{eq:fair_infoNCE}) objectives, we sample the positively-paired data from the joint distribution $P_{XY}$ and the negatively-paired data from the product of the conditional distributions $P_{X|Z}P_{Y|Z}$. For WeaklySup-InfoNCE (\eqref{eq:weaksup_infoNCE}) objective, we sample the positively-paired data from the product of the conditional distributions $P_{X|Z}P_{Y|Z}$ and the negatively-paired data from the product of the marginal distributions $P_{X}P_{Y}$. In a colloquial level, we can regard the pair of data $(x,y)$ sampled from $P_{XY}$ as strongly-correlated, such as variants of the same image by applying different image augmentations. We can regard the pair of data $(x,y)$ sampled from $P_{X|Z}P_{Y|Z}$ as two random data that are both associated with the same value of the conditioned variable, such as two random images that are both describing a blue object (by conditioning on the blue color). We car regard the pair of data $(x,y)$ sampled from $P_{X}P_{Y}$ as two random data, such as two random images. 

==> sec/archive/intro_old.tex <==
\section{Introduction}
Contrastive learning \citep{chopra2005learning, gutmann2010noise, oord2018representation} has become a prevalent approach for learning representations, with applications spanning learning self-supervised \citep{chen2020simple, he2020momentum}, weakly-supervised \citep{gupta2020contrastive, tsai2021integrating}, fair \citep{tsai2021conditional}, and supervised representations \citep{khosla2020supervised}. A contrastive objective like \citet{oord2018representation} is learning similar representations for \textit{positively-paired} data and dissimilar for \textit{negatively-paired} data. For instance, self-supervised learning define positive pair as blablabla {\color{olive} should we define in terms of computer vision, or in terms of general SSL} {\color{red} defining in terms of computer vision is simpler, but change the original citation from Oord et al. to SimCLR, and says that is is visual contrastive learning}, define negative pair as blablabla. {\color{olive} Could we replace the new genre with the fact that representation learned by SSL surpasses supervised counterparts in certain tasks?} {\color{red} we can get rid of new genre. But I don't think surpassing supervised counterparts is true. change it and build a transition to the next paragraph. }Recent literature shows that self-supervised learning opens a new genre of learning good representations even without access to downstream supervision.

Distinct contrastive literature adopts different constructions for positive and negative pairs \citep{chen2020simple, robinson2020contrastive, wu2020conditional, tsai2021integrating, tsai2021conditional, khosla2020supervised}. Among those constructions, the {\em conditional sampling procedure} plays an important role, where the conditional sampling procedure defines the data sampling process under certain conditions. As the first example, hard negative samples method~\citep{xxx} constructs the negatively-paired data by selecting random instances that are difficult to tell them apart. This work performs the sampling of negative pairs by conditioning on the distance between instances. As the second example, weakly-supervised method~\citep{tsai2021integrating} constructs the positively-paired data by selecting random instances with the same value of weak-supervision signals (e.g., Instagram images with same hashtags). This work performs the sampling of positive pairs by conditioning on the weak-supervision signals. As the third example, the fair contrastive method~\citep{tsai2021conditional} constructs the negatively-paired data by selecting random instances with the same value of sensitive information (e.g., gender information). This work performs the sampling of negative pairs by conditioning on the sensitive information.



paragraph 3: {\color{olive} Martin: Could we give a name of the limitation, like limited samples from conditional variable? Useful for later discussions} {\color{red} it's hard... But leave this comment here, I'll think of it when writing section 3}In this paper, we discuss a potential limitation in the conditional sampling procedure. A premise of the conditional sampling procedure is that dataset must exist sufficient samples that share a same value of the conditioned variable. From the following example, we will see how this premise raises the limitation. Assume that we select the conditioned variable to be the RGB color information, conditioning on the value of ``chalk white'' color. Then, the conditional sampling procedure requires us to sample a number of instances with the ``chalk white'' color. Nonetheless, since ``chalk white'' is not a common color, the datasets can contain insufficient samples with this color. This limitation is more obvious when the cardinality of the conditioned variable is large (contains lots of discrete attributes) or the conditioned variable is continuous. A work-around of this limitation is to perform clustering or quantizing the conditioned variable~\citep{tsai2021integrating} to ensure that each value of the conditioned variable correspond to sufficient samples in the dataset.  However, it is not optimal in the case that performing clustering or quantizing lose precision of the conditioned variable.


paragraph 4: We address the above limitation (the requirement of lots of empirical samples with a same value of the conditioned variable in the dataset) by leveraging a conditional generative model to perform conditional generation given the conditioned variable's value. {\color{olive} probably rewrite with fewer details?} {\color{red} sure, please do it.} Instead of training a separate conditional generative network like C-GANs~\citep{xxx}, we perform generation using the kernel conditional embedding operator~\citep{song2013kernel}, which contains no training parameters and its computation depends only on the kernel estimation of the conditional probability of the generative model. We further present a new contrastive learning framework by incorporating the kernel conditional mean operator. The new framework can work under the scenarios when we need to perform conditional sampling procedure but without sufficient empirical samples with a same value of the conditioned variable.

paragraph 5: We perform experiments blablabla. maybe after more details of the experiemnts, shall we start writing this paragraph.




==> sec/archive/method_old.tex <==
\section{Method}
% \subsection{Conditional Sampling using Kernel Conditional Embedding Operator}
\label{subsec:kernel_method}
Our goal is to convert the HardNeg-InfoNCE (\eqref{eq:hard_infoNCE}), WeaklySup-InfoNCE (\eqref{eq:weaksup_infoNCE}), and Fair-InfoNCE (\eqref{eq:fair_infoNCE}) objectives such that there is no need to sample from the conditional distributions to calculate these objectives. Precisely, without access to data pairs sampled from $P_{X|Z}P_{Y|Z}$, we still want to model these objectives given only the data: $\{(x_i, y_i, z_i)\}_{i=1}^b$, where $b$ is the batch size, and $\{(x_i, y_i, z_i)\}_{i=1}^b$ are independently sampled from the joint distribution $P_{XYZ}$. $(x_i, y_i, z_i)$ is from $P_{XYZ}$, because we can easily sample positively-paired data $(x_i, y_i) \sim P_{XY}$ (e.g., two augmented views of the same image), and by combining the associated conditional variable's outcome $z_i$ (e.g., the annotative attribute of the image), the triplet $(x_i, y_i, z_i)$ are samples from the joint distribution $P_{XYZ}$. Also, $y_j$ is not associated with $z_i$ whenever $j\neq i$, implying we cannot sample data of $Y$ from $P_{Y|Z}$ {\color{olive} could we expand the last sentence a bit more?}.
% Note that $\{z_i\}_{i=1}^b$ can all be different values. 

The intuition of our approach is to use a conditional generative model to model the conditional distribution $P_{Y|Z}$ based on $\{(x_i, y_i, z_i)\}_{i=1}^b \sim P_{XYZ}^{\,\,\,\otimes b}$. We use the kernel conditional embedding operator~\citep{song2013kernel} as the generative model, which uses kernel embedding statistics from $\{(x_i, y_i, z_i)\}_{i=1}^b$ to estimate the expected value of some kernel feature map under $P_{Y|Z}$. To begin with, we introduce the notations:
\paragraph{Notations.} We define $K_{XY}\in\mathbb{R}^{b\times b}$ as a kernel gram matrix between $X$ and $Y$. In specific, we let the $i_{\rm th}$ row and $j_{\rm th}$ column of $K_{XY}$ to be the exponential scoring function $e^{f(x_i, y_j)}$ (see~\eqref{eq:f}): $[K_{XY}]_{ij} := e^{f(x_i, y_j)}$. $K_{XY}$ is a gram matrix because the design of $e^{f(x, y)}$ satisfies a kernel between $g_{\theta_X}(x)$ and $g_{\theta_Y}(y)$:
$$
e^{f(x,y)} = {\rm exp}\,\bigg({\rm cosine\,\,similarity} \Big(g_{\theta_X}(x), g_{\theta_Y}(y)\Big) / \tau \bigg) := \bigg\langle \phi\Big(g_{\theta_X}(x)\Big), \phi\Big(g_{\theta_Y}(y)\Big) \bigg\rangle_{\mathcal{H}},
$$
where $\langle \cdot, \cdot \rangle_{\mathcal{H}}$ represents the inner product in a Reproducing Kernel Hilbert Space (RKHS) $\mathcal{H}$ with dimension $d$, $\phi$ is a feature map, $\phi\Big(g_{\theta_X}(x)\Big)$ is the kernel embedding of $x$, and $\phi\Big(g_{\theta_Y}(y)\Big)$ is the kernel embedding of $y$. Arranging in a vector form, we let $K_{XY} = \Phi_X\Phi_Y^{\top} \in \mathbb{R}^{b \times b}$ with $\Phi_X = \big[\phi\big(g_{\theta_X}(x_1)\big), \cdots, \phi\big(g_{\theta_X}(x_b)\big)\big]^\top$ and $\Phi_Y = \big[\phi\big(g_{\theta_Y}(y_1)\big), \cdots, \phi\big(g_{\theta_Y}(y_b)\big)\big]^\top$. To take the conditioning variable $Z$ into account, we define $K_{Z}\in \mathbb{R}^{b\times b}$ as a kernel gram matrix for $Z$. Specifically, we let $[K_Z]_{ij}$ to be the kernel similarity between $z_i$ and $z_j$: $[K_Z]_{ij} := \big\langle \gamma(z_i), \gamma(z_j) \big\rangle_{\mathcal{G}}$, with $\gamma(z)$ being the kernel embedding of $z$ and $\mathcal{G}$ being the associated RKHS space. Arranging in a vector form, we let $K_Z = \Gamma_Z \Gamma_Z^\top$ with $\Gamma_Z = \big[\gamma(z_1), \cdots , \gamma(z_b)\big]^\top$. 

Now we are ready to present the following lemma and our main results:


% From Martin: the discussion of Z is in later paragraphs

% {\color{red} Similarly}, we define $K_{Z}\in \mathbb{R}^{b\times b}$ as a kernel gram matrix for $Z$. In specific, we let $[K_Z]_{ij}$ to be the kernel similarity between $z_i$ and $z_j$: $[K_Z]_{ij} := \big\langle \gamma(z_i), \gamma(z_j) \big\rangle_{\mathcal{G}}$, with $\gamma(z)$ being the kernel embedding of $z$ and $\mathcal{G}$ being the associated RKHS space. Arranging in a vector form, we let $K_Z = \Gamma_Z \Gamma_Z^\top$ with $\Gamma_Z = \big[\gamma(z_1), \cdots , \gamma(z_b)\big]^\top$. {\color{red} hmmm, adding the discussion on $K_Z$ here? or maybe hinted why we need $K_Z$. and in the later paragraph, we discuss more on it. -> yeah maybe this is good. Since this is a notation section, just give it a very brief reason why we also want $K_Z$. And change the ``similarly''. There can be a much better transition for why we want $K_Z$}

%\paragraph{Overview.} Our method contains two steps. First, we observe that the the scoring function between a data pair ($f(x,y)$ in \eqref{eq:f}) can be understood as a particular kernel similarity. Next, we adopt a finite-samples kernel approximation for the scoring function between an anchor data $x$ and the data $y$ that is conditionally sampled from $P_{Y|Z=z}$ with $z$ being associated with $x$. In particular, instead of sampling $y$ from $P_{Y|Z=z}$, we generate conditional embedding of $y$ using kernel conditional embedding operator~\citep{song2013kernel}, then computing the scoring function between the anchor data $x$ and the generated conditional embedding. Since our method does not require sampling $y$ from $P_{Y|Z=z}$, we can overcome the limitation stated in Section~\ref{subsec:limitation} - when the dataset contains insufficient data of $Y$ that are associated with $z$.

\begin{lemma}[Kernel Conditional Embedding Operator~\citep{song2013kernel}]
The finite-sample kernel estimation of $\mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big]$ is $\hat{\mathcal{C}}_{Y|Z} \, \gamma (z) = \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \gamma (z)$ with $\hat{\mathcal{C}}_{Y|Z}$ being the kernel conditional embedding operator~\citep{song2013kernel}. 
\label{lemm:kernel_estimation}
\end{lemma}
{\color{red} some discussion}

\iffalse
\begin{corollary}
The estimation in Lemma~\ref{lemm:kernel_estimation} can be seen as applying the kernel smoothing technique~\citep{scholkopf2002learning}: $\mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big]\approx \sum_{j=1}^b \hat{p}(z_j| z)\, \phi\Big(g_{\theta_Y}(y_j)\Big)$ with $\hat{p}(z_j | z) = \sum_{k=1}^b \big[(K_Z + \lambda {\bf I})^{-1}\big]_{jk} \,\big\langle \gamma(z_k), \gamma(z) \big\rangle_{\mathcal{G}}$, since $\Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \gamma (z) = \sum_{j=1}^b \hat{p}(z_j| z)\, \phi\Big(g_{\theta_Y}(y_j)\Big)$.
\label{corollary:kernel_smoothing_phi}
\end{corollary}

{\color{red} this interpretation is terrible... change it when you woke up....} {\color{blue} A little help: $\Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \gamma (z) = \sum_{j=1}^b \hat{p}(z_j| z)\, \phi\Big(g_{\theta_Y}(y_j)\Big)$ with $\hat{p}(z_j | z) = \sum_{k=1}^b \big[(K_Z + \lambda {\bf I})^{-1}\big]_{jk} \,\big\langle \gamma(z_k), \gamma(z) \big\rangle_{\mathcal{G}}$. This can be regarded as applying kernel smoothing~\citep{scholkopf2002learning}. colloquial explanation: we weighted sum the embedding of $y_j$ via how predictable $z_j$ given $z$ and the predictability is determined by the kernel similarity (vague here, but basically this is what it is). In short, we estimate $\mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big]$ via $\sum_{j=1}^b \hat{p}(z_j| z)\, \phi\Big(g_{\theta_Y}(y_j)\Big)$. } Note that $\Phi_Y^{\top} \in \mathbb{R}^{d \times b}$ and $(K_Z + \lambda {\bf I})^{-1} \Gamma_Z \gamma (z) \in \mathbb{R}^{b \times 1}$. Row $i$ of $\hat{\mathcal{C}}_{Y|Z}$ corresponds to a weighted sum of row $i$ in  $\Phi_Y^{\top}$ with non-uniform weight $(K_Z + \lambda {\bf I})^{-1} \Gamma_Z \gamma (z)$ determined by the conditioning variable $Z$, reflecting the effect of conditioning on $Z$. 
Now, we are ready to present our main result:
\fi

\vspace{1mm}
\begin{proposition}[Estimation of $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$] Given $\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}$, we can estimate $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$ as $\Big[ K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z \Big]_{ii}$.
\label{prop:main_result}
\end{proposition}
\begin{proof} First, for any $Z=z$, along with Lemma~\ref{lemm:kernel_estimation}, we estimate $\phi\Big(g_{\theta_Y}(y)\Big)$ when $y\sim P_{Y|Z=z}$:
$$
\phi\Big(g_{\theta_Y}(y)\Big) \,\,{\rm when}\,\, y\sim P_{Y|Z=z} \approx \mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big] \approx \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z). 
$$
Then, we plug in the result for the data pair $(x_i, z_i)$ to estimate $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$:
\begin{equation*}
\begin{split}
    & \bigg\langle \phi\Big(g_{\theta_X}(x_i)\Big), \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z_i) \bigg\rangle_{\mathcal{H}} = {\rm tr} \bigg( \phi\Big(g_{\theta_X}(x_i)\Big)^\top \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z_i)\bigg) \\
    =  \,\,& [K_{XY}]_{{\rm row}\,i} (K_Z + \lambda {\bf I})^{-1} [K_{Z}]_{{\rm column}\,i}
    = \Big[ K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z \Big]_{ii}.
\end{split}
\end{equation*}
\end{proof}

{\color{red} some discussion}

\begin{corollary}
The estimation in Proposition~\ref{prop:main_result} can be re-formulated as $\Big[ K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z \Big]_{ii} = \sum_{j=1}^b \hat{p}(z_j|z_i)\, e^{f(x_i, y_j)}$ with $\hat{p}(z_j | z_i) = \sum_{k=1}^b \big[(K_Z + \lambda {\bf I})^{-1}\big]_{jk} \,\big\langle \gamma(z_k), \gamma(z_i) \big\rangle_{\mathcal{G}}$. Thehe reformulation can be seen as applying the kernel smoothing technique~\citep{scholkopf2002learning} for the estimation: 
\vspace{-3mm}
$$e^{f(x_i,y)} \,\,{\rm when}\,\, y\sim P_{Y|Z=z_i} \approxapprox \sum_{j=1}^b \hat{p}(z_j|z_i)\, e^{f(x_i, y_j)}.$$
\label{coro:kernel_smoothing_exp_scoring}
\end{corollary}

{\color{blue} colloquial explanation: we weighted sum via how predictable $z_j$ given $z_i$ and the predictability is determined by the kernel similarity (vague here, but basically this is what it is).}


{\color{olive} Intepretation of $K_Z$ here, as discussed Sep 27, the re-weighted sum}
Proposition~\ref{prop:main_result} leverages the kernel conditional embedding operator~\citep{song2013kernel} as a conditional generative model that generates the conditional embedding of $Y$ (i.e., $\mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big]$) when conditioning on $Z=z$. Using the kernel conditional embedding operator has the advantages of not 1) requiring sampling $y\sim P_{Y|Z=z}$, alleviating the limitation of having insufficient data of $Y$ that are associated with $z$; 2) generating raw data directly; and 3) including additional training parameters.


{\color{red} rephrasing the following interpretation as a discussion for this Proposition. Can shorten the discussion on $K_{XY}$, and put more emphasis on discussing $K_Z$. Focus on discuss $K_{XY}$, $K_Z$, and then the whole proposition 3 }


We start by discussing $K_{XY}$, where $[K_{XY}]_{ij} = e^{f(x_i, y_j)}$. Since $\{(x_i, y_i, z_i)\}_{i=1}^b$ are independently sampled from $P_{XYZ}$, $(x_i, y_j)$ are sampled from $P_{XY}$ when $i=j$ and from $P_{X}P_{Y}$ when $i\neq j$. That is, the kernel gram matrix $K_{XY}$ has its on-diagonal entries representing the similarities between the data pair sampled from $P_{XY}$ and its off-diagonal entries representing the similarities between the data pair sampled from $P_XP_Y$.


Next, we discuss $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$. $[K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z]_{ii}$ is the kernel estimation of $e^{f(x_i, y)}$ when $(x_i,z_i)\sim P_{XZ}\,,\,y\sim P_{Y|Z=z_i}$. Hence, the on-diagonal entries of $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$ defines the similarity between the data pair sampled from $P_{X|Z}P_{Y|Z}$. In a colloquial level, we can view $(K_Z + \lambda {\bf I})^{-1} K_Z$ as a transformation applied on $K_{XY}$, converting unconditional similarity measurements between $X$ and $Y$ to conditional similarity measurements. In the rest of the paper, we short hand $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$ as $K_{X\indep Y|Z}$, following prior work~\citep{fukumizu2007kernel} that short hands $P_{X|Z}P_{Y|Z}$ as $P_{X\indep Y|Z}$.

Last, we discuss $K_Z$. Note that $K_Z$ defines the kernel similarities among $\{z_i\}_{i=1}^b$, and we have flexibility to arbitrarily design $K_Z$. {\color{red} Add more discussions and examples here.}

\paragraph{Converting Existing Contrastive Learning Objectives.} Now, we reintroduce the original WeaklySup-InfoNCE (\eqref{eq:weaksup_infoNCE}), Fair-InfoNCE (\eqref{eq:fair_infoNCE}), and HardNeg-InfoNCE (\eqref{eq:hard_infoNCE}) objectives with our discussed kernel expression. Recall that $K_{XY}$ is blablabla and $K_{X\indep Y|Z}$ is blablabla.
\begin{equation}
{\rm {WeaklySup}_{Kernel}} := \mathbb{E}_{\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}}\Big[\frac{1}{b}\sum_{i=1}^b {\rm log}\,\frac{[K_{X\indep Y|Z}]_{ii}}{[K_{X\indep Y|Z}]_{ii} + \sum_{j\neq i} [K_{XY}]_{ij}}\Big].
\label{eq:weaksup_kernel}
\end{equation}
\begin{equation}
{\rm {Fair}_{Kernel}} :=\mathbb{E}_{\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}}\Big[\frac{1}{b}\sum_{i=1}^b {\rm log}\,\frac{[K_{XY}]_{ii}}{[K_{XY}]_{ii} + (b-1) [K_{X\indep Y|Z}]_{ii}}\Big].
\label{eq:fair_kernel}
\end{equation}
\begin{equation}
{\rm {HardNeg}_{Kernel}} :=\mathbb{E}_{\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}}\Big[\frac{1}{b}\sum_{i=1}^b {\rm log}\,\frac{[K_{XY}]_{ii}}{[K_{XY}]_{ii} + (b-1) [K_{X\indep Y|Z}]_{ii}}\Big].
\label{eq:hardneg_kernel}
\end{equation}






==> sec/archive/method_older.tex <==
\section{Method}


\subsection{Conditional Sampling using Kernel Conditional Embedding Operator}
\label{subsec:kernel_method}

Our goal is to convert the HardNeg-InfoNCE (\eqref{eq:hard_infoNCE}), WeaklySup-InfoNCE (\eqref{eq:weaksup_infoNCE}), and Fair-InfoNCE (\eqref{eq:fair_infoNCE}) objectives such that, within these objectives, there is no need to sample data of $Y$ from $P_{Y|Z}$. Precisely, without access to data pairs sampled from $P_{X|Z}P_{Y|Z}$, we still want to model these objectives given only a batch of positively-paired data as well as its associated conditional variable's value: $\{(x_i, y_i, z_i)\}_{i=1}^b$, where $b$ is the batch size and $\{(x_i, y_i, z_i)\}_{i=1}^b$ are independently sampled from $P_{XYZ}$. Note that $\{z_i\}_{i=1}^b$ can all be different values. Under this situation, from this batch, $y_j$ is not associated with $z_i$ whenever $j\neq i$, implying we cannot sample data of $Y$ from $P_{Y|Z}$.


The intuition of our approach is to leverage a conditional generative model, which relies on $\{(x_i, y_i, z_i)\}_{i=1}^b \sim P_{XYZ}^{\,\,\,\otimes b}$, to model the conditional distribution $P_{Y|Z}$. We consider the conditional generative model using the kernel conditional embedding operator~\citep{song2013kernel}, which is computed via kernel statistics from $\{(x_i, y_i, z_i)\}_{i=1}^b$. To begin with, we introduce the notations.

\paragraph{Notations.} We define $K_{XY}\in\mathbb{R}^{b\times b}$ as a kernel gram matrix between $X$ and $Y$. In specific, we let the $i_{\rm th}$ row and $j_{\rm th}$ column of $K_{XY}$ to be the exponential scoring function $e^{f(x_i, y_j)}$ (see~\eqref{eq:f}): $[K_{XY}]_{ij} := e^{f(x_i, y_j)}$. The reason why $K_{XY}$ has a kernel expression is because the design of $e^{f(x, y)}$ admits a kernel similarity between $g_{\theta_X}(x)$ and $g_{\theta_Y}(y)$:
$$
e^{f(x,y)} = {\rm exp}\,\bigg({\rm cosine\,\,similarity} \Big(g_{\theta_X}(x), g_{\theta_Y}(y)\Big) / \tau \bigg) := \bigg\langle \phi\Big(g_{\theta_X}(x)\Big), \phi\Big(g_{\theta_Y}(y)\Big) \bigg\rangle_{\mathcal{H}},
$$
where $\langle \cdot, \cdot \rangle_{\mathcal{H}}$ represents the inner product in a Reproducing Kernel Hilbert Space (RKHS) $\mathcal{H}$, $\phi$ is the associated feature mapping in $\mathcal{H}$, $\phi\Big(g_{\theta_X}(x)\Big)$ is the kernel embedding of $x$, and $\phi\Big(g_{\theta_Y}(y)\Big)$ is the kernel embedding of $y$. Arranging in a vector form, we let $K_{XY} = \Phi_X\Phi_Y^{\top}$ with $\Phi_X = \big[\phi\big(g_{\theta_X}(x_1)\big), \cdots, \phi\big(g_{\theta_X}(x_b)\big)\big]^\top$ and $\Phi_Y = \big[\phi\big(g_{\theta_Y}(y_1)\big), \cdots, \phi\big(g_{\theta_Y}(y_b)\big)\big]^\top$. Similarly, we define $K_{Z}\in \mathbb{R}^{b\times b}$ as a kernel gram matrix for $Z$. In specific, we let $[K_Z]_{ij}$ to be the kernel similarity between $z_i$ and $z_j$: $[K_Z]_{ij} := \big\langle \gamma(z_i), \gamma(z_j) \big\rangle_{\mathcal{G}}$, with $\gamma(z)$ being the kernel embedding of $z$ and $\mathcal{G}$ being the associated RKHS space. Arranging in a vector form, we let $K_Z = \Gamma_Z \Gamma_Z^\top$ with $\Gamma_Z = \big[\gamma(z_1), \cdots , \gamma(z_b)\big]^\top$. Now, we present our main result:

%\paragraph{Overview.} Our method contains two steps. First, we observe that the the scoring function between a data pair ($f(x,y)$ in \eqref{eq:f}) can be understood as a particular kernel similarity. Next, we adopt a finite-samples kernel approximation for the scoring function between an anchor data $x$ and the data $y$ that is conditionally sampled from $P_{Y|Z=z}$ with $z$ being associated with $x$. In particular, instead of sampling $y$ from $P_{Y|Z=z}$, we generate conditional embedding of $y$ using kernel conditional embedding operator~\citep{song2013kernel}, then computing the scoring function between the anchor data $x$ and the generated conditional embedding. Since our method does not require sampling $y$ from $P_{Y|Z=z}$, we can overcome the limitation stated in Section~\ref{subsec:limitation} - when the dataset contains insufficient data of $Y$ that are associated with $z$.

\vspace{1mm}
\begin{proposition}[Finite-Samples Kernel Estimation of $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$] Given a batch of samples $\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}$, using the kernel conditional embedding operator~\citep{song2013kernel}, the finite-samples kernel estimation of $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$ is $\Big[ K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z \Big]_{ii}$.
\label{prop:main_result}
\end{proposition}
\begin{proof} First, for any $Z=z$, we estimate $\phi\Big(g_{\theta_Y}(y)\Big)$ when $y\sim P_{Y|Z=z}$ via the following:
$$
\phi\Big(g_{\theta_Y}(y)\Big) \,\,{\rm when}\,\, y\sim P_{Y|Z=z} \approx \mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big] \approx \hat{\mathcal{C}}_{Y|Z} \, \gamma (z) = \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z).
$$
$\hat{\mathcal{C}}_{Y|Z}$ is the kernel conditional embedding operator~\citep{song2013kernel} with $\hat{\mathcal{C}}_{Y|Z} :=  \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z$. 
Then, we plug in the result for the data pair $(x_i, z_i)$ to estimate $e^{f(x_i,y)}$ when $y\sim P_{Y|Z=z_i}$:
\begin{equation*}
\begin{split}
    & \bigg\langle \phi\Big(g_{\theta_X}(x_i)\Big), \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z_i) \bigg\rangle_{\mathcal{H}} = {\rm tr} \bigg( \phi\Big(g_{\theta_X}(x_i)\Big)^\top \Phi_Y^\top (K_Z + \lambda {\bf I})^{-1} \Gamma_Z \, \gamma(z_i)\bigg) \\
    =  \,\,& {\rm tr} \bigg( [K_{XY}]_{{\rm row}\,i} (K_Z + \lambda {\bf I})^{-1} [K_{Z}]_{{\rm column}\,i}\bigg)
    = \Big[ K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z \Big]_{ii}.
\end{split}
\end{equation*}
\end{proof}

Proposition~\ref{prop:main_result} leverages the kernel conditional embedding operator~\citep{song2013kernel} as a conditional generative model that takes in an embedding of $Z$ (i.e., $\gamma(z)$) and output an embedding of $Y$ (i.e., $\mathbb{E}_{y\sim P_{Y|Z=z}}\Big[\phi\Big(g_{\theta_Y}(y)\Big)\Big]$). Using the kernel conditional embedding operator has the advantages of not 1) requiring sampling $y\sim P_{Y|Z=z}$, alleviating the limitation of having insufficient data of $Y$ that are associated with $z$; 2) generating raw data directly; and 3) including additional training parameters.



\paragraph{Interpretation.}

We start by discussing $K_{XY}$, where $[K_{XY}]_{ij} = e^{f(x_i, y_j)}$. Since $\{(x_i, y_i, z_i)\}_{i=1}^b$ are independently sampled from $P_{XYZ}$, $(x_i, y_j)$ are sampled from $P_{XY}$ when $i=j$ and from $P_{X}P_{Y}$ when $i\neq j$. That is, the kernel gram matrix $K_{XY}$ has its on-diagonal entries representing the similarities between the data pair sampled from $P_{XY}$ and its off-diagonal entries representing the similarities between the data pair sampled from $P_XP_Y$.

Next, we discuss $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$. $[K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z]_{ii}$ is the kernel estimation of $e^{f(x_i, y)}$ when $(x_i,z_i)\sim P_{XZ}\,,\,y\sim P_{Y|Z=z_i}$. Hence, the on-diagonal entries of $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$ defines the similarity between the data pair sampled from $P_{X|Z}P_{Y|Z}$. In a colloquial level, we can view $(K_Z + \lambda {\bf I})^{-1} K_Z$ as a transformation applied on $K_{XY}$, converting unconditional similarity measurements between $X$ and $Y$ to conditional similarity measurements. In the rest of the paper, we short hand $K_{XY} (K_Z + \lambda {\bf I})^{-1} K_Z$ as $K_{X\indep Y|Z}$, following prior work~\citep{fukumizu2007kernel} that short hands $P_{X|Z}P_{Y|Z}$ as $P_{X\indep Y|Z}$.

Last, we discuss $K_Z$. Note that $K_Z$ defines the kernel similarities among $\{z_i\}_{i=1}^b$, and we have flexibility to arbitrarily design $K_Z$. {\color{red} Add more discussions and examples here.}

\paragraph{Converting Existing Contrastive Learning Objectives.} Now, we convert the HardNeg-InfoNCE (\eqref{eq:hard_infoNCE}), WeaklySup-InfoNCE (\eqref{eq:weaksup_infoNCE}), and Fair-InfoNCE (\eqref{eq:fair_infoNCE}) objectives with the discussed kernel expression.  

The converted HardNeg-InfoNCE and  Fair-InfoNCE objectives would be
$$
\mathbb{E}_{\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}}\Big[\frac{1}{b}\sum_{i=1}^b {\rm log}\,\frac{[K_{XY}]_{ii}}{[K_{XY}]_{ii} + (b-1) [K_{X\indep Y|Z}]_{ii}}\Big].
$$

The converted WeaklySup-InfoNCE objective would be
\begin{align}
    \mathbb{E}_{\{(x_i, y_i, z_i)\}_{i=1}^b\sim P_{XYZ}^{\,\,\,\otimes b}}\Big[\frac{1}{b}\sum_{i=1}^b {\rm log}\,\frac{[K_{X\indep Y|Z}]_{ii}}{[K_{X\indep Y|Z}]_{ii} + \sum_{j\neq i} [K_{XY}]_{ij}}\Big]. \label{eq:weakinfonce}
\end{align}





==> sec/archive/unused.tex <==
\section{Old Introduction}

Contrastive representation learning~\citep{chen2020simple,he2020momentum,khosla2020supervised} has recently attracted lots of attention, and its objective is to learn similar representations for data that are {\em positively-paired} and dissimilar representations for data that are {\em negatively-paired}. For instance, self-supervised visual contrastive approaches~\citep{chen2020simple,he2020momentum} consider augmented variants (i.e., applying image augmentations) of the same image to be positively-paired and different images as negatively-paired. It is worth noting that self-supervised contrastive approaches require no access to downstream tasks' supervision and serve as strong representation pre-training baselines. In addition to applying the aforementioned constructions for positive and negative data pairs, other contrastive learning work adopts different constructions, resulting in distinct applications, such as learning wealy-supervised~\citep{tsai2021integrating}, fair~\citep{tsai2021conditional}, and supervised~\citep{khosla2020supervised} representations. For example, weakly-supervised contrastive approaches~\citep{tsai2021integrating} consider data with same auxiliary information (e.g., Instagram images that share the same image hashtags) to be positively-paired and data with different auxiliary information as negatively-paired.


We can realize the positive and negative pairs construction via {\em sampling procedure from data distributions}. In our first example, the self-supervised contrastive approaches~\citep{oord2018representation,tsai2021self,bachman2019learning,hjelm2018learning} suggest that for positively-paired $x$ and $y$, since they are augmented variants of the same data, they can be seen as different views to each other, as if they are sampling from the joint distribution of the data: $(x,y) \sim P_{XY}$. On the contrary, for negatively-paired data $x$ and $y$, since they are different data, they are regarded as sampling from the product of marginal distributions: $(x,y) \sim P_XP_Y$. Note that $X$ and $Y$ are identically distributed and $P_X$ and $P_Y$ represent the data distribution. In our second example, the weakly-supervised contrastive approaches~\citep{tsai2021integrating} suggest that positively-paired $x$ and $y$ will share the same auxiliary information. If representing $Z$ as the variable of auxiliary information and $z$ to be its value, then the positive pair are regarded as sampling from the product of conditional distributions: $(x,y) \sim P_{X|Z=z}P_{Y|Z=z}$. As the third example, the fair contrastive approaches~\citep{tsai2021conditional} constructs the negative data pairs $(x,y)\sim P_{X|Z=z}P_{Y|Z=z}$ when treating $Z$ as the sensitive variable such as ``gender'' and $z$ as the value of it such as ``male''. In short, distinct contrastive approaches admit different sampling procedures to construct positive and negative pairs.

Various sampling procedures in contrastive learning literature can be potentially unified in a {\em conditional sampling} form: $(x,y)\sim P_{X|Z}P_{Y|Z}$. To see this, $P_{X|Z}P_{Y|Z}$ specializes to $P_{XY}$ when treating $Z$ as instance-ID, specializes to $P_XP_Y$ when treating $Z$ as a null variable, and varies in different applications when treating $Z$ as different variables (e.g., auxiliary information~\citep{tsai2021integrating}, sensitive information~\citep{tsai2021conditional}).

Not only does this form expand flexibility , it also reminds us potential challenges





%and fair contrastive approaches~\citep{tsai2021conditional} define a positive pair as augmented variants of the same data and a negative pair as random data with the same value of the conditioned variable (e.g., we can select the conditioned variable to be sensitive information such as gender). 



%as uncorrelated ; and supervised contrastive approaches~\citep{khosla2020supervised} considers data with the same downstream label as correlated and data with different downstream labels as uncorrelated. 


Human annotated labels can be expensive and time-consuming to collect. Self-supervised learning (\textbf{SSL}) aims to learn useful representations without human annotated labels, by obtaining supervision signals from the data itself \citep{facebookai}. A prominent way of SSL is contrastive learning \citep{chen2020simple}, which uses contrastive objectives \citep{gutmann2010noise, oord2018representation} to guide a representation encoder $f$ to pull together embeddings from similar samples (termed as \textbf{positive} pairs) closer, and push away embedding from dissimilar samples (termed as \textbf{negative} pairs) further \citep{khosla2020supervised, robinson2020contrastive}. Representations learned by contrastive SSL have shown better performances than their supervised counterparts for transfer learning in certain
cases \citep{chen2021empirical}.

% Despite strong performances in downstream tasks, current contrastive SSL methods often do not discuss how to incorporate or remove specific information in the representation. This is important because of two reasons: 1) the representation learned from SSL method may contain undesirable information, such as gender or race bias, which we want to remove. 2) If additional information are provided with the data, such as the hashtags as auxiliary attributes for Instagram image, it can also provide valuable (and maybe noisy, thus weak) supervision when learning the representation via SSL. 

Recent works \citep{robinson2020contrastive, wu2020conditional, tsai2021integrating,tsai2021conditional} have proposed methods which we summarize as \textbf{conditional} sampling framework in contrastive SSL. This framework is very useful: ~\citet{wu2020conditional} and \citet{robinson2020contrastive} sample negative pairs conditionally to avoid easy, uninformative examples, and improve downstream performances in a variety of tasks. \citet{tsai2021integrating} samples positive pairs conditionally to incorporate auxiliary information (e.g., additional attributes from the dataset) in the SSL representation, and \citet{tsai2021conditional} samples negative pairs conditionally to remove sensitive information like gender or age in the SSL representation.


The goal is to incorporate or remove information in the SSL representation. The idea is to create a conditional variable $Z$ which is related to the attributes or information we want to incorporate or remove. ~\citet{tsai2021integrating} samples positive pairs \citep{tsai2021integrating} from data that share the same $z$ to incorporate information, meanwhile \citep{tsai2021conditional} samples negative pairs from data that share the same $z$ to remove information.





\paragraph{to be dissected into later sub-sections.}
To demonstrate that our method can generalize to the three major conditional sampling scheme in Self-Supervised Learning, we perform experiments on 4 existed datasets and create a new ColorMNIST dataset to support the validation experiments of Fair-InfoNCE. We first describe the 4 existed datasets used in the experiments: 

{\bf 1) CIFAR10} \cite{krizhevsky2009learning}: It contains 60000 32x32 color images spanning 10 classes. Each image is center aligned common object in the real world, e.g. automobile / plane / dog. {\bf 2) ImageNet-100}~\cite{russakovsky2015imagenet}: It's a subset of ImageNet-1k~\cite{russakovsky2015imagenet} for image classification task, where 100 categories out of 1000 are selected, resulting in 0.12 million images. {\bf 3) UT-Zappos}~\cite{yu2014fine} This dataset contains 50,025 shoes images defined over 21 categories. Each image is annotated with 7 discrete attributes as auxiliary information. To simplify conditioning process, we expand each attribute into multiple binary attributes, which results in total 128 binary attributes. {\bf 4) CUB-200-2011 } \cite{wah2011caltech}: 11,788 bird images spanning 200 fine-grain bird species are included in this dataset, meanwhile 312 binary attributes are attached to each image. 


{\bf 5) ColorMNIST}: ColorMNIST is a dataset we create in this paper to demonstrate how to remove continuous variable during contrastive learning pretraining. We assign a continuous RBG color value to each training image in the Yann LeCun's version of MNIST dataset~\cite{lecun1998gradient} (hand writing digits and rescaled to 32x32) as its background color. By design, the background color we are adding has superficial correlation with the class label. With this superfical correlation, networks are prone to overfitting. In our later section, we will demonstrate that with the help of our kernel conditional embedding operator, contrastive learning performed on this dataset can remove the bias of background colors, suggesting a promising way of tackling fairness problem in contrastive learning. An example of the created training images are demonstrated in Figure~\ref{fig:colormnist-img}.

\input{fig_tex/colorMNIST}



\subsection{Old - Weakly Supervised Contrastive Learning}
\label{subsec:old_weaksup_contrastive}
The kernel conditional embedding operator allows us to approximate the conditional sampling process without perform the sampling itself. Here, we first demonstrate its superiority for incorporating high dimensional auxiliary information into contrastive pretraining (WeaklySup-InfoNCE, Equation~\ref{eq:weakinfonce}). Three datasets are considered here: {\bf UT-Zappos, CUB-200-2011, ImageNet-100}. 
\paragraph{Condition on High Dimensional Discrete Variable} For {\bf UT-Zappos}, we consider 128 dimensional attributes variables, each of which covers a certain feature of shoes. For {\bf CUB-200-2011}, 312 binary attributes are used, each of which highlights specific aspect of a bird image (e.g. red hawk). Note that UT-Zappos and CUB-200-2011 naturally has high dimensional discrete features to condition upon. Although informative, the high dimension variable makes the conditional sampling process very challenging. In {\bf CUB-200-2011}, for example, if we consider the latent variable $Z$ as a 312 dimensional binary variable, then performing conditional sampling from $Z$ requires access sufficient amount of data for each $Z$ configuration. However, for the entire CUB-200-2011 dataset, there's only on average 1.001 data point per $Z$ configuration, hence there's might not be enough data to support the conditional sampling process. 

\paragraph{Condition on Continuous Variable} 
Although it's difficult to perform condition sampling based on high dimensional discrete variables, it is statistically impossible to do the same for continuous variable. One work around would be to perform discretization of the continuous variables, but it would lose information undesirably. Our method, on the other hand, avoid directly performing conditional sampling process while still effectively approximate the conditioning sampling statistics in the contrastive learning objective, making it more suitable for conditioning on continuous variables. To support this claim, we choose ImageNet-100 dataset with its corresponding features (512 dimension) extracted by OpenAI-CLIP encoder (ResNet-50 Architecture). 


\paragraph{Kernel Choice and Performance Gain}
Out of various kernel settings we experiment with, we find the linear kernel works the best (i.e. use f(x) = x as the kernel function) for WeakSup-InfoNCE setting. Results of other kernels can be found in the Appendix. To demonstrate our method has unique advantages when conditioning on high-dim/continuous variables, we compare it with previous Cl-InfoNCE method. Although Cl-InfoNCE shows consistent improvement upon baseline {\it unconditional} method (SimCLR), the additional information's strength hasn't been fully utilized due to the poor sampling process. Our method, on the other hand, shows consistent advantages over Cl-InfoNCE based on linear evaluation protocal. {\color{red} discuss the Best results of Cl-InfoNCE v.s. using all attributes}
\input{tbl_tex/cl_infonce}


\subsection{Old - Fair Contrastive Learning}
\label{subsec:old_fair_contrastive}
Another application of conditional sampling lies in removing data bias from learnt representations. To the extreme case, it's devastating if contrastive pretraining find a short cut that only exploit the dataset bias in the training set for the downstream task. Not only could it impair the the generalization ability of the model, but also could rise concerns about privacy, equality and fairness when deployed to the real world. Hence, there's 2 main objectives to test the performance of Fair-InfoNCE: {\bf 1) Generalization error}: whether the learnt representation can still be useful on the new data. ({\color{red} Currently the testing set is also colored and color is class-related, maybe we should change it to color but class unrelated.}) {\bf 2) Bias removal}: How much bias information still remains in the learnt representation. With the ColorMNIST created, we guage the performance of the model under these two objectives.



Practically speaking, while generalization error is represented via Linear evaluation protocals, the bias removal performance can be measured in a similar fashion. We train a linear read-out layer $h(\cdot)$ that maps the learnt representation to RGB color of the image background, supervised by the ground truth RGB background color value. We use Mean Square Error (MSE) between the prediction and ground truth as the training objective for $h(\cdot)$ and also the testing MSE as the final performance measurement. Larger testing MSE score would indicate a more successful bias removal. 

{\color{red} Add discretization for colorMNIST exp using c-infonce}
\input{tbl_tex/fair_infonce}
For training details, we employ LeNet-5~\cite{lecun1998gradient} as the backbone architecture. Images are resized to 32x32 and batch size of training is set to be 1024. We train both the baseline (unconditional) SimCLR and our model for 1000 gradient descent steps while early stopping is applied to prevent further overfitting. For our kernel conditional embedding operator, we choose a non-linear kernel defined as follows:
\[
\displaystyle f(x) = \begin{cases} 
 |x|  & \text{if $ -0.5 \leq x \leq 0.5$}\\  
 1 & \text{otherwise} 
 \end{cases} 
\]

The results of Table~\ref{tbl:fair-infonce} shows the comparsion between Fair-InfoNCE and the baseline SimCLR. We can observe that via using the kernel conditional embedding operator, we are able partially remove the bias information (background color) from the learnt representation as when regressing by the same protocal, the MSE testing error is larger than that of unconditional SimCLR meanwhile the linear classification read-out (generalization) is improved.


\subsection{Old - Hard-Negatives Contrastive Learning}
\label{subsec:old_hardneg_contrastive}
The last application in contrastive learning we include here is to show case that our method can also approximate the conditional sampling process during hard negative mining. As discussed in Section \ref{method:hardnegatives}, hard negative mining can make contrastive learning more efficient. We use {\bf CIFAR10} and {\bf ImageNet-100} to demonstrate our method can achieve state-of-the-art hard negative mining performance meanwhile maintain the high flexiblity of mining criterion. We adopt two kernels for this part of the study: (i) $f_{\text{thresholding}}$ (ii) $f_{\text{trapezoid}}$, which are defined as follows:

\[
\displaystyle f_{\text{thresholding}}(x) = \begin{cases} 
 1  & \text{if $ t_1 \leq |x| \leq t_2$}\\  
 0 & \text{otherwise} 
 \end{cases} 
\]

\[
\displaystyle f_{\text{trapezoid}}(x) = \begin{cases} 
 1  & \text{if $ t_1 \leq |x| \leq t_2$}\\  
 |x| & \text{otherwise} 
 \end{cases} 
\]

We use Resnet-50 as base encoder for both dataset. LARS optimizer are used. For CIFAR10, we train the pre-training stage for 400 epochs with 256 batch size and for ImageNet-100, we choose 512 batch size for pre-training 200 epochs. Note that the batch size for ImageNet-100 here is different from that used in WeaklySup-InfoNCE (Section~\ref{rsl:weaksup}) to compensate the fact that HardNeg-InfoNCE is purely self-supervised whereas Section~\ref{rsl:weaksup} are incorporating addition information. 


From Table~\ref{tbl:hardnegatives} we can see that our method yields competitive results comparing to the state-of-the-art hard negative mining procedures~\cite{robinson2020contrastive} in both small and large batch size settings. However, unlike other hard negative mining schemes which adopt separate procedures, we can simplify the control of different hard negative mining criterion via customizing the kernel function $f(\cdot)$ of $K_Z$. This allows experimenting with different hard negative mining schemes without changing the majority of the loss code base, hence can allow faster developmental cycles, which is valuable especially when time and efficiency are priority concerns. 

\input{tbl_tex/hard_negatives}

\subsection{Ablation on kernel choice}
\input{tbl_tex/ablation_kernels}

==> submission_supple.tex <==

% \documentclass{article} % For LaTeX2e
% \usepackage{iclr2022_conference,times}

% % Optional math commands from https://github.com/goodfeli/dlbook_notation.
% \input{math_commands.tex}


% \usepackage{float}

% \usepackage{wrapfig}

% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2021}

% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2021}

% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2021}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{xcolor}         % colors

% \hypersetup{
%     colorlinks = true,
%     linkbordercolor = {white},
%     citecolor={olive}
% }

% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{multirow}
% \usepackage[ruled,vlined]{algorithm2e}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}

% \title{Appendix for Conditional Contrastive Learning with Kernel}
% % Authors must not appear in the submitted version. They should be hidden
% % as long as the \iclrfinalcopy macro remains commented out below.
% % Non-anonymous submissions will be rejected without review.

% \author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
% about author (webpage, alternative address)---\emph{not} for acknowledging
% funding agencies.  Funding acknowledgements go at the end of the paper.} \\
% Department of Computer Science\\
% Cranberry-Lemon University\\
% Pittsburgh, PA 15213, USA \\
% \texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
% \And
% Ji Q. Ren \& Yevgeny LeNet \\
% Department of Computational Neuroscience \\
% University of the Witwatersrand \\
% Joburg, South Africa \\
% \texttt{\{robot,net\}@wits.ac.za} \\
% \AND
% Coauthor \\
% Affiliation \\
% Address \\
% \texttt{email}
% }

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to \LaTeX{} to determine where to break
% % the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% % puts 3 of 4 authors names on the first line, and the last on the second
% % line, try using \AND instead of \And before the third author name.

% \newcommand{\fix}{\marginpar{FIX}}
% \newcommand{\new}{\marginpar{NEW}}

% %\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
% \begin{document}


% \maketitle
% \appendix

% \input{sec/appendix}

% \newpage


% \bibliography{ref}
% \bibliographystyle{iclr2022_conference}

% \end{document}


==> tbl_tex/ablation_kernels.tex <==

\begin{table}[t!]
\vspace{-2mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|cc}
\toprule
Method              & \textbf{Linear Evaluation} \\ \midrule \midrule 
SimCLR (unconditional)~\citep{chen2020simple}      & 77.8 $\pm$ 1.5                     \\ \midrule  
Cl-InfoNCE~\citep{tsai2021integrating}      & 84.6 $\pm$ 0.4                             \\  \midrule
Ours - RBF kernel      &R6 $\pm$               \\ \midrule
Ours - polynomial kernel      & R5 $\pm$               \\ \midrule
Ours - linear kernel      & R4 $\pm$               \\ \midrule 
Ours - cosine kernel      & \textbf{86.6} $\pm$ 0.3                \\ \midrule 
 \midrule 

\end{tabular}
}
\vspace{-1mm}
\caption{\small Ablation Study on different kernel functions using UT-Zappos datasets}
\label{tbl:ablation-kernels}
\vspace{-1mm}
\end{table}

==> tbl_tex/cl_infonce.tex <==

\begin{table}[t!]
\vspace{-2mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|cccc}
\toprule
Method              & \textbf{UT-Zappos}& \textbf{CUB} &\textbf{ImageNet-100}\\ \midrule \midrule 
SimCLR~\citep{chen2020simple}      & 77.8 $\pm$ 1.5               & 14.1 $\pm$ 0.7          & 76.2 $\pm$ 0.3 \\ \midrule \midrule 
Cl-InfoNCE (optimal)~\citep{tsai2021integrating}      & 84.6 $\pm$ 0.4               & 20.6 $\pm$ 0.5          & 81.4 $\pm$ 0.4 \\ \midrule \midrule 
Cl-InfoNCE (raw)~\citep{tsai2021integrating}      & 82 $\pm$ -                & 19 $\pm$ -          & 73 $\pm$ - (2500 clusters)\\ \midrule \midrule 
Ours & \textbf{86.6} $\pm$ 0.3              & \textbf{29.9} $\pm$0.3             & \textbf{82.4} $\pm$ 0.5\\ \midrule \midrule 

\end{tabular}
}
\vspace{-1mm}
\caption{\small Experiments WeaklySup-InfoNCE. Note that the batch size of ImageNet-100 is 128.}
\label{tbl:cl-infonce-results}
\vspace{-1mm}
\end{table}

==> tbl_tex/fair_infonce.tex <==

\begin{table}[t!]
\vspace{-2mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|ccc}
\toprule
Method              & \textbf{Linear Evaluation}& \textbf{MSE score} \\ \midrule \midrule 
SimCLR~\citep{chen2020simple}      & 93.9 $\pm$ 0.3               & 3.2 $\pm$ 0.8          \\ \midrule \midrule 
Ours (thresholding) & \textbf{95.2} $\pm$ 0.4              & \textbf{9.1} $\pm$1.4             \\ \midrule \midrule 
Ours (cosine kernel) & R1 $\pm$ -              & R1 $\pm$ -          \\ \midrule \midrule 

\end{tabular}
}
\vspace{-1mm}
\caption{\small Experiments on ColorMNIST. Linear evaluation and }
\label{tbl:fair-infonce}
\vspace{-1mm}
\end{table}

==> tbl_tex/hard_negatives.tex <==

\begin{table}[t!]
\vspace{-2mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|ccc}
\toprule
Method              & \textbf{CIFAR-10} & \textbf{ImageNet-100} \\ \midrule \midrule 
SimCLR (unconditional)~\citep{chen2020simple}      & 89.9 $\pm$ 0.2               & 77.8 $\pm$ 0.4          \\ \midrule \midrule 
Hard Negative~\citep{robinson2020contrastive}      & 91.4 $\pm$ 0.2                & 79.2 $\pm$ 0.5                 \\ \midrule \midrule 
Kernel Conditional Embedding (ours, thresholding kernel)      & 91.6 $\pm$ 0.1                & \textbf{80.6} $\pm$ 0.6                 \\ \midrule \midrule 
Kernel Conditional Embedding (ours, trapezoid kernel) & 91.5 $\pm$ 0.2               & 79.8 $\pm$ 0.5              \\ \midrule \midrule 
Kernel Conditional Embedding (ours, cosine kernel) & R2 $\pm$ -              & R3 $\pm$ -             \\ \midrule \midrule 
\end{tabular}
}
\vspace{-1mm}
\caption{\small Experiments of sampling hard negatives. Note that the batch size of ImageNet-100 is 512.}
\label{tbl:hardnegatives}
\vspace{-1mm}
\end{table}
